Complexity of limit cycles with block-sequential update schedules in conjunctive networks

In this paper, we deal the following decision problem: given a conjunctive Boolean network defined by its interaction digraph, does it have a limit cycle of a given length k? We prove that this problem is NP-complete in general if k is a parameter of the problem and in P if the interaction digraph is strongly connected. The case where $k$ is a constant, but the interaction digraph is not strongly connected remains open. Furthermore, we study the variation of the decision problem: given a conjunctive Boolean network, does there exist a block-sequential (resp. sequential) update schedule such that there exists a limit cycle of length k? We prove that this problem is NP-complete for any constant k >= 2.

==> cycles_3_6.tex <==
\begin{tikzpicture}[node distance=2cm]
\setlength{\radio}{5cm}
%\setlength{\radio}{3cm}
\node[main node] (x1) {$1$};
\node[main node, right of=x1] (x2) {$2$};
\node[main node, below of=x2] (x3) {$3$};
\node[main node, below of=x1] (x4) {$4$};
\node[main node, below right of=x1,xshift=-0.4cm,yshift=0.4cm] (x5) {$5$};

\path[arcos]
(x1) edge (x2)
(x2) edge (x3)
(x3) edge (x4)
(x4) edge (x1)
(x1) edge (x5)
(x5) edge (x2)
(x3) edge (x5)
(x5) edge (x4)
;
\end{tikzpicture}

